Efficient Replication of Queued Tasks for Latency Reduction in Cloud Systems

In cloud computing systems, assigning a job to multiple servers and waiting for the earliest copy to finish is an effective method to combat the variability in response time of individual servers. Although adding redundant replicas always reduces service time, the total computing time spent per job may be higher, thus increasing waiting time in queue. The total time spent per job is also proportional to the cost of computing resources. We analyze how different redundancy strategies, for eg. number of replicas, and the time when they are issued and canceled, affect the latency and computing cost. We get the insight that the log-concavity of the service time distribution is a key factor in determining whether adding redundancy reduces latency and cost. If the service distribution is log-convex, then adding maximum redundancy reduces both latency and cost. And if it is log-concave, then having fewer replicas and canceling the redundant requests early is more effective.

==> GJ_macros.tex <==
\newcommand{\TODO}[1]{\todo[color=blue!25, inline]{ TODO: #1} \index{To Do: !#1}}

\newtheorem{lem}{Lemma}
\newtheorem{thm}{Theorem}
\newtheorem{defn}{Definition}
\newtheorem{coro}{Corollary}
\newtheorem{clm}{Claim}
\newtheorem{conj}{Conjecture}
\newtheorem{exple}{Example}
\newtheorem{prop}{Proposition}
\newtheorem{propty}{Property}
\newtheorem{rem}{Remark}

\newcommand{\E}[1]{\mathbb{E}\left[{#1}\right]}
\newcommand{\V}[1]{\mathrm{Var}\left[{#1}\right]}
\newcommand{\posfunc}[1]{\lvert {#1}\rvert ^{+}}
\newcommand{\HyperExp}{\textit{HyperExp}}
\newcommand{\SExp}{\textit{ShiftedExp}}
\newcommand{\Pareto}{\textit{Pareto}}
\newcommand{\xor}{\oplus}
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\graphicspath{{Figures/}}


\crefname{equation}{}{}
\Crefname{equation}{}{}
\crefname{thm}{theorem}{theorems}
\Crefname{thm}{Theorem}{Theorems}
\crefname{clm}{claim}{claims}
\Crefname{clm}{Claim}{Claims}
\Crefname{coro}{Corollary}{Corollaries}
\Crefname{lem}{Lemma}{Lemmas}
\Crefname{sec}{Section}{Sections}
\crefname{app}{appendix}{appendices}
\Crefname{app}{Appendix}{Appendices}
\crefname{prop}{proposition}{propositions}
\Crefname{prop}{Proposition}{Propositions}
\Crefname{propty}{Property}{Properties}
\crefname{figure}{fig.}{figures}
\Crefname{figure}{Fig.}{Figures}
\crefname{defn}{definition}{definitions}
\Crefname{defn}{Definition}{Definitions}
\crefname{fact}{fact}{facts}
\Crefname{fact}{Fact}{Facts}
\crefname{appendix}{appendix}{appendices}
\Crefname{appendix}{Appendix}{Appendices}
\crefname{algo}{algorithm}{algorithms}
\Crefname{algo}{Algorithm}{Algorithms}
\crefname{algorithm}{algorithm}{algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefname{conj}{conjecture}{conjectures}
\Crefname{conj}{Conjecture}{Conjectures}
\crefname{obs}{observation}{observations}
\Crefname{obs}{Observation}{Observations}

==> rep_partial_forking_v2__Gauri_Joshi_s_conflicted_copy_2015-05-26_.tex <==
% %% IN THIS VERSION WE REPLACE LIGHT-EVERYWHERE BY LOG-CONCAVE 

We now analyze the latency-cost trade-off for the $(n,r,k)$ partial fork-join system where, instead of forking a job to all $n$ servers, an incoming job it is forked to some $r$ servers according to a symmetric forking policy (\Cref{defn:symmetric_forking}). Some examples of symmetric forking policies are:
\begin{enumerate}
\item \textit{Group-based random: } This policy holds when $r$ divides $n$. The $n$ servers are divided into $n/r$ groups of $r$ servers each. A job is forked to one of these groups, chosen uniformly at random. 
\item \textit{Uniform Random: } A job is forked to any $r$ out of $n$ servers, chosen uniformly at random.
\item \textit{Partial Cancellation: } A job is forked to all $n$ servers. As soon as $r$ of them start service, the remaining tasks are canceled. This is equivalent to having a centralized queue and forking to the first $r$ servers that become idle.
\end{enumerate}

%\subsection{Partial Forking}
%\label{subsec:rep_partial_fork}
\subsection{Latency-Cost Analysis}

The key property of a scheduling policy that affects the latency-cost performance is that relative starting times of the tasks of a job. Staggered task start times can save the computing cost $\E{C}$, but could cause a loss of diversity resulting in higher latency $\E{T}$. In a group-based policy, all the $r$ tasks of a job start service at the same instant. As a result it is simple to derive exact expressions for latency and cost as given in \Cref{lem:latency_cost_group_based} below.
\begin{lem}
\label{lem:latency_cost_group_based}
The latency and cost of the group-based random policy where each job is forked to one of $n/r$ groups of servers are given by
\begin{align}
\E{T} &= \E{X_{1:r}}  + \frac{\lambda r \E{X_{1:r}^2}}{2(n - \lambda r \E{X_{1:r}})} \label{eqn:E_T_group_based} \\
\E{C} &= r \E{X_{1:r}} \label{eqn:E_C_group_based}
\end{align}
\end{lem}

To prove \Cref{lem:latency_cost_group_based} observe that each group behaves like an independent $(r,1)$ fork-join system with Poisson arrivals at rate $\lambda r/n$, whose latency and cost is given by \Cref{thm:rep_queueing}. For other symmetric forking policies, it is difficult to get an exact analysis of $\E{T}$ and $\E{C}$ because the tasks of a job can start at different times. However, we can get bounds on $\E{C}$ depending on the log-concavity of $X$, given in \Cref{thm:E_C_r_trend} below.

\begin{thm}
\label{thm:E_C_r_trend}
Consider an $(n,r,1)$ partial-fork join system, with a symmetric forking policy. In the extreme cases $r=1$ and $r = n$, $\E{C} = \E{X}$ and $\E{C} = n \E{X_{1:n}}$ respectively. For $1 < r <n$, we get bounds on $\E{C}$ depending on the tail of $X$,
\begin{align} 
 r \E{X_{1:r}} \geq \E{C} &\geq \E{X} \quad \quad \text{if } \bar{F}_X \text{ is  log-concave} \\
\E{X} \geq \E{C} &\geq r \E{X_{1:r}}  \quad \text{if } \bar{F}_X \text{ is  log-convex}
\end{align} 
\end{thm}

The proof of \Cref{thm:E_C_r_trend} is given in Appendix~\ref{sec:rep_queueing_proofs}. In the sequel, we use the bounds given by \Cref{thm:E_C_r_trend} to gain insights into choosing the best $r$ and best scheduling policy when $\bar{F}_X$ is log-concave or log-convex.

\subsection{Choosing the optimal $r$}
When the arrival rate $\lambda$ small, the latency is dominated by the service time $\E{X_{1:r}}$ which is non-increasing in $r$. This can be observed for the group-based forking policy by taking $\lambda \rightarrow 0$ in \eqref{eqn:E_T_group_based}. Thus we get the following result.

\begin{lem}[Latency vs $r$ in low load regime]
\label{lem:latency_low_lambda}
Forking to all $n$ servers, that is, $r =n$ gives the lowest latency in the low $\lambda$ regime for any service time distribution $F_X$. 
\end{lem}

We use the computing cost $\E{C}$ to compare systems with different $r$ in the high $\lambda$ regime. Using \eqref{eqn:E_C_group_based} and \Cref{clm:capacity_in_terms_of_EC}, we can infer that the service capacity (maximum supported $\lambda$) for an $(n,r,1)$ system with group-based random forking is
\begin{align}
\lambda_{max} = \frac{n}{r\E{X_{1:r}}}
\end{align}

By \Cref{propty:r_E_X_1_r_trend} in Appendix~\ref{sec:tail_properties} we know that the cost $\E{C} = r \E{X_{1:r}}$ is non-decreasing with $r$ for log-concave $\bar{F}_X$, and is non-increasing for log-convex $\bar{F}_X$. Thus $r=1$ ($r= n$) gives the highest service capacity for log-concave (log-convex) $\bar{F}_X$. The system with highest service capacity also gives lowest latency in the high $\lambda$ regime. 

For other symmetric forking policies, we can use \Cref{thm:E_C_r_trend} together with \Cref{clm:capacity_in_terms_of_EC} to get the following corollaries comparing different $r$ in the high traffic regime.

\begin{coro}[Service Capacity vs. $r$]
\label{coro:serv_capacity_r}
In the $(n,r,1)$ partial fork-join system, $r=1$ ($r=n$) gives the highest service capacity for log-concave (log-convex) $\bar{F}_X$. 
\end{coro}

\begin{coro}[Latency vs. $r$ in high traffic regime]
\label{coro:optimal_r}
Given the number of servers $n$, and symmetric forking of each job to $r$ servers, if $\bar{F}_X$ is log-concave (log-convex) , $r=1$ ($r=n$) gives lowest latency $\E{T}$ in the high traffic (high $\lambda$) regime. 
\end{coro}

\Cref{coro:optimal_r} was previously proven in \cite{shah_when_2013} using a combinatorial argument. But using $\E{C}$, we get an alternate, and arguably simpler way to prove the same result. \Cref{coro:serv_capacity_r} and \Cref{coro:optimal_r} are illustrated by Fig.~\ref{fig:E_T_rep_shifted_exp_vs_lambda_diff_r} and Fig.~\ref{fig:E_T_rep_hyper_exp_vs_lambda_diff_r} where latency $\E{T}$ is plotted versus $\lambda$ for different values of $r$. In \Cref{fig:E_T_rep_shifted_exp_vs_lambda_diff_r} the service time distribution is $\SExp(\Delta, \mu)$ (which is log-concave) with $\Delta = 1$ and $\mu = 0.5$. When $\lambda$ is small, more redundancy (higher $r$) gives lower latency, but in the high $\lambda$ regime, $r=1$ gives lowest latency and highest service capacity. On the other hand in Fig.~\ref{fig:E_T_rep_hyper_exp_vs_lambda_diff_r}, for a log-convex distribution $\HyperExp(p, \mu_1, \mu_2)$, in the high load regime the latency decreases as $r$ increases.

\begin{figure}[t]
\centering
\includegraphics[width=3.25in]{E_T_rep_shifted_exp_vs_lambda_diff_r.pdf}
\caption{For $X \sim \SExp(1,0.5)$ which is log-concave, forking to less (more) servers reduces latency in the low (high) $\lambda$ regime. Each job is assigned to $r$ servers chosen uniformly at random from $n = 6$ servers. \label{fig:E_T_rep_shifted_exp_vs_lambda_diff_r}}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=3.25in]{E_T_rep_hyper_exp_vs_lambda_diff_r.pdf}
\caption{For $X \sim \HyperExp(p, \mu_1, \mu_2)$ with $p=0.1$, $\mu_1 = 1.5$, and $\mu_2 = 0.5$ which is log-convex, forking to more servers (larger $r$) gives lower latency for all $\lambda$. Each job is assigned to $r$ servers chosen uniformly at random from $n = 6$ servers.  \label{fig:E_T_rep_hyper_exp_vs_lambda_diff_r}}
\end{figure}

\Cref{lem:latency_low_lambda} and \Cref{coro:optimal_r} imply that forking to more servers (larger $r$) gives lower latency in the low $\lambda$ and high $\lambda$ regimes. But we observe in \Cref{fig:E_T_rep_hyper_exp_vs_lambda_diff_r} that this true for all $\lambda$. 

\begin{conj}[Optimality for log-convex $F_X$]
\label{conj:opt_heavy_tail}
For log-convex $F_X$ and any arrival rate $\lambda$, forking a job to all $n$ servers is optimal in both $\E{T}$ and $\E{C}$.
\end{conj}

From \eqref{eqn:E_T_group_based} we can show that \Cref{conj:opt_heavy_tail} is true for the group-based forking policy. But the proof for other symmetric forking policies remains open.

\begin{figure}[t]
\centering
\includegraphics[width=3.25in]{E_T_shifted_exp_vs_lambda_diff_policies.pdf}
\caption{For service distribution $\SExp(1, 0.5)$ which is log-concave, uniform random scheduling (which staggers relative task start times) gives lower latency than group-based random for all $\lambda$. The system parameters are $n= 6$, $r=2$. \label{fig:E_T_shifted_exp_vs_lambda_diff_policies}}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=3.25in]{E_T_hyper_exp_vs_lambda_diff_policies.pdf}
\caption{ For service distribution $\HyperExp(0.1, 1.5, 0.5)$ which is log-convex, group-based scheduling gives lower latency than uniform random in the high $\lambda$ regime. The system parameters are $n= 6$, $r=2$. \label{fig:E_T_hyper_exp_vs_lambda_diff_policies}}
\end{figure}

\subsection{Choosing the Scheduling Policy}
For a given $r$, we now compare different policies of choosing the $r$ servers for each job, e.g. group-based random, uniform random etc. \Cref{clm:capacity_in_terms_of_EC} implies that for a given $n$ and $r$, the symmetric forking policy that results in a higher $\E{C}$ has higher latency $\E{T}$ in the high $\lambda$ regime. The $\E{C}$ for a given scheduling policy depends on the relative starting times of the $r$ tasks at queues. 

%The starting times affect $\E{C}$ in two opposing ways:
%\begin{enumerate}
%\item If the starting times are staggered such that some of them are cancelled before starting service, we can save on the computing cost $\E{C}$.
%\item But having fewer tasks running simultaneously results in loss of diversity, resulting in a larger $\E{C}$.
%\end{enumerate}
%
%The first factor dominates for log-concave $\bar{F}_X$,  distributions, the second dominates for log-convex distributions. 
For the group-based policy in which all $r$ tasks start simultaneously, $\E{C} = r \E{X_{1:r}}$ from \eqref{eqn:E_C_group_based}. By \Cref{thm:E_C_r_trend} we know that $\E{C} \geq r \E{X_{1:r}}$ for log-convex $\bar{F}_X$. This implies that staggering the task start times does not help. Similarly, for log-concave $\bar{F}_X$, since $\E{C} \leq r \E{X_{1:r}}$, a forking policy with higher diversity in the relative starting times of tasks gives lower latency. We state this formally is \Cref{coro:optimal_policy} below.

\begin{coro}
\label{coro:optimal_policy}
For a given $n$ and $r$, and task arrival distribution at each queue, if $\bar{F}_X$ is log-concave (log-convex), the symmetric forking policy which results in more diversity in the relative task start times gives lower (higher) latencyin the high $\lambda$ regime.
\end{coro}

This phenomenon is illustrated in Fig.~\ref{fig:E_T_hyper_exp_vs_lambda_diff_policies} and Fig.~\ref{fig:E_T_shifted_exp_vs_lambda_diff_policies} for the uniform random and group-based random policies. Uniform random policy gives more diversity in relative start times than the group-based random policy. The task arrivals at each queue are Poisson with rate $\lambda r/n$ for both policies. 


%For log-concave distributions, we can use \Cref{lem:any_load_ET_EC} and \Cref{thm:E_C_r_trend} to infer that a scheduling policy that staggers the relative task service start times gives lower latency. Hence we can get the following corollary. %This does not directly follow from \Cref{lem:any_load_ET_EC} and \Cref{thm:E_C_r_trend}, but we can show it for the shifted exponential distribution in \Cref{lem:shifted_exp_opt_sched} below. 
%
%\begin{coro}
%\label{coro:log_concave_opt_sched}
%For log-concave $X$, uniform random scheduling gives lower latency than the group-based forking policy. 
%\end{coro}

%In Fig.~\ref{fig:E_T_rep_shifted_exp_vs_lambda_diff_policies} we compare the latency versus $\lambda$ for different scheduling polcies. 

%\Cref{lem:rep_partial_fork_SExp_bound} below shows that for the shifted exponential distribution (light tailed), the latency of random scheduling is lower than group-based policy. And the inequality hold even for cases when $r$ does not divide $n$.
%
%\begin{lem}[Upper bound for $\SExp(\Delta, \mu)$]
%\label{lem:rep_partial_fork_SExp_bound}
%For service distribution $\SExp(\Delta, \mu)$, the latency and cost with partial forking to $r$ out of $n$ servers, chosen uniformly at random are bounded as follows
%\begin{align}
%\E{T} &\leq \Delta + \frac{1}{r \mu}  + \frac{\lambda r( (\Delta + \frac{1}{r \mu})^2 + \frac{1}{r^2 \mu^2})}{2(n - \lambda r(\Delta + \frac{1}{r \mu}))} \label{eqn:E_T_partial_fork_bnd} \\
%\E{C} &\leq r \Delta + \frac{1}{\mu} %\\
%%\E{N} &= r
%\end{align}
%\end{lem}
%
%Fig.~\ref{fig:E_T_rep_shifted_exp_vs_r} we plot the latency $\E{T}$ versus $r$ for $\SExp(1, 0.5)$, and its upper bound given by \Cref{lem:rep_partial_fork_SExp_bound}. The bound is tight for $r=1$ and $r=n$, and loose for intermediate $r$. This is due to the staggered relative times of tasks of a job with the random scheduling. Also, we note the bound is more loose for larger $\Delta$.

%\begin{proof}[Proof of \Cref{lem:rep_partial_fork_SExp_bound}]
%First consider the cases where $n$ is divisible by $r$. Let the partial forking system where a job is forked to $r$ randomly chosen servers be referred to as System $1$. Consider System $2$ where the $n$ servers are divided into fixed groups of $r$ servers each. In System $2$, each job is forked to the $r$ servers in a randomly chosen group. Observe that in both systems the average arrival rate to each server is equal to $\lambda r/n$. The difference is the System $2$ follows a stricter group-based assignment of tasks of a job. We compare these two systems and use System $2$ to upper bound the performance of System $1$ for shifted exponential service time.
%
%In System $2$, all $r$ tasks of a job start service at the same time, and as soon as one task finishes the others are cancelled.  Thus, each group in System $2$ is equivalent to an $M/G/1$ queue with Poisson arrival rate $\lambda r/n$ with service distribution $\E{X_{1:r}}$. The mean response time of an $M/G/1$ queueing system can be found using the Pollaczek-Khinchine formula and is equal to the upper bound expression in \eqref{eqn:E_T_partial_fork_bnd}. The total time spent by the servers on each job is equal to $\E{C}^{(2)} = r \E{X_{1:r}} = r \Delta + 1/\mu$. 
%
%In System $1$, the $r$ tasks of a job are assigned to $r$ randomly chosen queues, without fixing groups of servers. Thus, the $r$ tasks of a job may not start service at the same time. Let their service start times be $t_1$, $t_2, \cdots t_r$ where $t_1 = 0$ without loss of generality. Let $S$ be the time between the start of service of the first task to reach head of its queue, and when any one of the $r$ tasks finishes. Then,
%\begin{align}
%S &=  \Delta + \min (Y_1, Y_2, \cdots Y_r) \\
%&= \Delta + W
%\end{align}
%where $Y_i \sim \SExp(t_i, \mu)$.  The tail distribution is given by,
%\begin{align}
%\Pr(W > w) &= 
%\begin{cases}
%e^{-\mu w} & 0 \leq w < t_2 \\
%e^{\mu t_2 -2\mu w} & t_2 \leq w < t_3 \\
%%e^{\mu (t_2 + t_3) - 3 \mu w } & t_3 \leq w < t_4 \\
%\vdots \\
%e^{\mu (t_2 + \cdots t_{r-1}) - (r-1) \mu w } & t_{r-1} \leq w < t_r \\
%e^{\mu (t_2 + \cdots t_{r}) - r \mu w } & t_{r} \leq w
% \end{cases}
%\end{align}
%
%The computing cost, or the time spent by the $n$ servers on each job is
%\begin{align}
%C^{(1)} &= S + \posfunc{ S - t_2} + \cdots + \posfunc{S - t_r} \\
%&= \Delta + W+ \posfunc{\Delta +W - t_2} + \cdots + \posfunc{\Delta +W- t_r} \\
%&\leq r\Delta + W+ \posfunc{W - t_2} + \cdots + \posfunc{W- t_r}
%\end{align}
%
%Taking expectation on both sides we get
%\begin{align}
%\E{C}^{(1)} &\leq r \Delta + \int_{0}^{\infty} \Pr(W >w) dw + \int_{t_2}^{\infty} \Pr(W >w) dw  \nonumber \\
%&\quad \quad \quad + \cdots  + \int_{t_r}^{\infty} \Pr(W >w) dw \\
%&= r \Delta +  \frac{1}{\mu}
%\end{align}
%
%
%Thus, the expected time spent on each job is smaller in System $1$ than System $2$, for the same number of servers and same overall arrival rate. As a result, the expected latency in System $1$ will be smaller than System $2$. The proof can be directly extended to the case where $n$ is not divisible by $r$.
%\end{proof}

%\begin{figure}[t]
%\centering
%\includegraphics[width=3.25in]{E_T_rep_shifted_exp_vs_r.pdf}
%\caption{Latency $\E{T}$ versus $r$, the number of servers each job is forked to, also proportional to the network cost. The total number of servers $n = 10$. The arrival rate is $\lambda = 0.25$ and service distribution is Shifted exponential with $\Delta = 1, 2$, $\mu = 0.5$. The upper bound is tight for $r=1$ and $r= n$. It gets more loose as $\Delta$ increases. \label{fig:E_T_rep_shifted_exp_vs_r}}
%\end{figure}

%\TODO{Explain the two partial forking plots in text}

%\TODO{Compare with Mor's setup: more generally $x$ classes of jobs being assigned to $r$ servers each using different policies}
